Document-Level Supervision for Multi-Aspect Sentiment Analysis Without Fine-grained Labels

Aspect-based sentiment analysis (ABSA) is a widely studied topic, most often trained through supervision from human annotations of opinionated texts. These fine-grained annotations include identifying aspects towards which a user expresses their sentiment, and their associated polarities (aspect-based sentiments). Such fine-grained annotations can be expensive and often infeasible to obtain in real-world settings. There is, however, an abundance of scenarios where user-generated text contains an overall sentiment, such as a rating of 1-5 in user reviews or user-generated feedback, which may be leveraged for this task. In this paper, we propose a VAE-based topic modeling approach that performs ABSA using document-level supervision and without requiring fine-grained labels for either aspects or sentiments. Our approach allows for the detection of multiple aspects in a document, thereby allowing for the possibility of reasoning about how sentiment expressed through multiple aspects comes together to form an observable overall document-level sentiment. We demonstrate results on two benchmark datasets from two different domains, significantly outperforming a state-of-the-art baseline.

==> future_work.tex <==
Our work has proposed a novel task for unsupervised aspect-based sentiment analysis which relaxes the assumption that a sentence will only have a single aspect. While this work has explored the possibility of training on full review documents and testing on individual sentences with multiple aspect-based sentiment annotations, further work could explore inference on complete documents allowing the greater contextual processing of the pretrained transformer language model to come to bear. Likewise existing baselines such as JASen \cite{huang-etal-2020-weakly} could be modified to fully explore their potential within the multi-aspect task.
